Saturn's ancient regular satellites

Are Saturn's regular satellites young or old? And how old are Enceladus' cratered plains? To answer these questions we computed model surface ages of the most heavily cratered terrains on Saturn's regular icy satellites using new high-resolution outer Solar System evolution simulations, and coupled with improved estimates of the trans-Neptunian objects populations. The output of the simulations allowed us to construct a model impact chronology onto Saturn which automatically applies to its regular satellites. We used crater densities and our impact chronology onto Saturn to construct model impact-crater isochrons, i.e., the scaling of the satellite crater production function with time. The surface ages derived for the cratered plains on Mimas, Enceladus, Tethys, Dione and Rhea range from 4.1 Ga to 4.4 Ga, with the surfaces of Mimas and Enceladus roughly 200 Myr younger than those of the outer three satellites. Uncertainties in these ages are less than 300 Myr. The calculated model surface ages of these satellites are consistent over as much as two orders of magnitude in the observed crater diameter. The similarity of the crater production function amongst all satellites suggests that they were bombarded by a single impactor source. This work supports the idea that Saturn's regular satellites are ancient, and has implications for their formation and their tidal evolution.

==> update.tex <==
\section{New way to calculate the age}
\label{sec:update}

\subsection{Decay profile of collision onto the planets}
\textit{First}, based on the results of the scattered disk simulations, we constructed the decay profiles of the collision onto each planets and the profiles with
$log|ln (1-F(t))| = \beta \log{\tau} - \beta \log{t}$ in the Weibull plot (lower-left of figure~\ref{fig:jup}, \ref{fig:sat}, and \ref{fig:ura}). 
This expression is the alternative form of the cumulative Weibull distribution, $F(t)=1-\exp{[(t/\tau)^{\beta}]}$, after taking a natural logarithm and logarithm in base of 10. (Weibull distribution, also known as stretched exponential function or Kohlrausch function) \\ 

For Jovian, Saturnian and Uranian system, we fitted the collisions onto the corresponding host planets after $300~$Myrs, $100~$Myrs, and $200~$Myrs of simulations. The fitting ranges are determined by trial for the best fit (judge by eyes). The reason for not fitting throughout the entire ranges is because, \textit{(1)} the rapid decline in the first few Myrs causes the curve drops from infinity, thus the calculated impact flux or the estimated crater densities of the very early time ($<~100~$Myr) to be unreasonably high; and \textit{(2)} large amount of data in the beginning skew the fit toward the early time of the simulation, and biases against the later time ( the recent period when counting backward in time, as the age of the solar system). \\

In table~\ref{tab:fit}, we list the fitting results. Given the in-completed simulations and the insufficiency of impacts onto Saturn, we use the average $\tau$ and $\beta$ of the collision onto Jupiter and Uranus to model the decay profile of Saturnian system for this time. At current, we have been running additional "Clones" simulations, which the initial condition of the planetesimals are cloned from the state vectors of the planetesimals at 1 Gyr of the scattered disc simulation. The results from "Clone" aims to improve the impact resolution after the giant migration and extend the cratering chronology to more recent time. \\

\begin{table*}[h!]
    \centering
    \begin{tabular}{l|ccc|ccc} \\
\textbf{System} & \textbf{SD fit ranges} & \textbf{$\tau_{\rm SD}$} & \textbf{$\beta_{\rm SD}$} & \textbf{Wong 2021 fit ranges}  & \textbf{$\tau_{\rm W21}$}& \textbf{$\beta_{\rm W21}$} \\
{\color[HTML]{666666} \textit{Unit}} & {\color[HTML]{666666} \textit{Myrs}} & {\color[HTML]{666666} \textit{Myrs}} & {\color[HTML]{666666} \textit{/}} & {\color[HTML]{666666} \textit{Myrs}} & {\color[HTML]{666666} \textit{Myrs}} & \multicolumn{1}{l}{{\color[HTML]{666666} \textit{}}} \\
 \hline \\
Jovian & 300  & 0.477& 0.263 & & 2.70 & 0.33 \\
Saturnian & 100  & 2.252& 0.343 & & 2.51 & 0.35 \\
\begin{tabular}[c]{@{}l@{}}Saturnian\\ (Average from\\ Jovian and Uranian)\end{tabular} & / & 0.602& 0.268 & & / & \\
Uranian& 200  & 0.726 & 0.272 & & 3.43 & 0.36 \\
Neptunian & 100  & 1.915 & 0.327 & & 1.80 & 0.32 \\
Combined  & 200  & 0.730 & 0.280 & \multirow{-6}{*}{32} & 2.58 & 0.35        
\end{tabular}
    \caption{}
    \label{tab:fit}
\end{table*}

\begin{figure*}[ht]
    \centering
    \resizebox{\hsize}{!}{\includegraphics{extra_fig/jup_efit300myr.png}}
    \caption{The normalized decay profile of the collision onto Jupiter based on the results of the scattered disk simulations. We express the flux of impact in logarithm scale (base of 10) in upper-left, and also express the time (in Myr) in the same logarithm scale in the upper-right. The lower-left is the Weibull plot showing all the data, and lower-right is the same plot but zooms into t~$>$~10 Myr. From the Weibull plot, we fit the data after 300 Myrs using the Weibull distribution, and to determine the e-folding time ($\tau$) and the stretching parameter ($\beta$) as $0.477~\pm??$~Myrs and $0.263~\pm~??$ respectively.}
    \label{fig:jup}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \resizebox{\hsize}{!}{\includegraphics{extra_fig/sat_efit100myr.png}}
    \caption{Similar as Fig.~\ref{fig:jup}, but plotting and fitting with the collisions onto Saturn. The best fit for the data after 100 Myrs using the Weibull distribution gives $\tau$ =~2.252~Myr and $\beta$ =~0.343. Compared to the collision on Jupiter and Uranus, there are not much on Saturn. Not having high confidence in the latest fitting of Saturn's collision, we adopt the $\tau$ an $\beta$ as those average from Jupiter's and Uranus' for now. We shall update the fitting and calculate once more simulations are completed.}
    \label{fig:sat}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \resizebox{\hsize}{!}{\includegraphics{extra_fig/ura_efit200myr.png}}
    \caption{Similar as Fig.~\ref{fig:jup}, but plotting and fitting with the collision onto Uranus. The best fit for the data after 200 Myrs using the Weibull distribution gives $\tau$ =~0.726~Myr and $\beta$ =~0.272. }
    \label{fig:ura}
\end{figure*}

The normalized cumulative impacts rate could be estimated based on the decay profile. By differentiating the cumulative Weibull distribution with time, for a specific time (t) in Myrs, the rate is,
\begin{equation*}
\frac{dF(t)}{dt}~=~\beta~\tau^{-\beta}~t^{\beta-1}~e^{-(t/\tau)^{\beta}}    
\end{equation*}
The $\beta$ and $\tau$ for each planet-satellites system is known from the former fitting. 
When $t=4500~$Myr (into the simulation), which arrives at the present time, the normalized cumulative impact on Saturn is $dF(t=4500)/dt~=~1.179 \times 10^{-8}$ per Myr, or $1.179 \times 10^{-14}$ per year. That would be the rate at present, and we will later deduce the rate and resultant number of impact backward in time. 
To get the actual rate of impact at present, we need to calculate the leakage rate from the scatter disk and the total number of scatter disk objects.

%=====================================================

\subsection{Impact rates onto the satellites}
\textit{Second}, we rely on the incoming flux of ecliptic comet ($F_{\rm EC}$) to estimate the impact flux onto each satellites. 
$F_{\rm EC}$ is computed by rate of decline of the scattered disk ($r_{\rm SD}$) and current number of scattered disk objects for a certain size ($N_{\rm SD}$). Expressed as $F_{\rm EC}~=~r_{\rm SD}~\times~N_{\rm SD}$. 
$r_{\rm SD}$~=~0.133 based on our scattered disk simulation results (for outer-edge of the disc at 31 AU or 33 AU); $N_{\rm SD}$ is 200 million, the number of objects with diameter (D)~$>$~10 km currently as computed by \citet{Nesvorny2019}.\\

We specify the size of the objects because the final crater's diameter depends on the size of the impactor, and the number of scattered disk object changes with their size. We estimated the crater densities of crater with various final crater sizes: $D_{\rm f}~>$~1 km, 2 km, 5 km, 10 km, and 20 km, on the satellites' surface, and compared with the corresponding observed crater densities from \citep{Kirchoff2009, KirchoffSchenk2010}.\\

To find out the size that an impactor requires to excavate a final crater of the above sizes, we used the crater scaling law from $\citet{Zahnle2003}$ ($\pi$-scaling law). 
To translate from the population of current scattered disk object with D~$>10$~km (200 million; from \citet{Nesvorny2019}) to the population with the required sizes, we applied the size-frequency distribution from \citet{Singer2019} and \citet{Nesvorny2016}, which suggested N(D$~<~1~\rm km)~\approx~\rm D^{0.7}$ and N(1$~\rm km~<~\rm D<~10~\rm km)~\approx~D^{3}$, respectively. 
The above two steps compute the $N_{\rm SD}$ that is large enough to create a certain size craters if they hit the satellites, and further calculate the $F_{\rm EC}$ of those objects. \\

As demonstration, on the surface of Enceladus, a satellite in the Saturnian system, with a final crater size of 20~km.
The size of impactors' diameter ($D_{\rm i}$) required is 0.88 km and the estimated population that is larger than such diameter is $2.191~\times~10^{9}$, that is the $N_{\rm SD}$ for this case. We have,
\begin{eqnarray*}
F_{\rm EC} &=& N_{\rm SD}~\times~r_{\rm SD}
           &=& (2.191 \times 10^{9})~\times~(0.133/\rm Gyr)
           &=& 0.291/\rm year
\end{eqnarray*}

We further multiple $F_{\rm EC}$ with the impact probability on Enceladus: $P_{\rm s}~=~4.34~\times~10^{-8}$, to reduce the incoming flux and consider only those that strike on Enceladus. Thus the rate of impact is :
$dN_{D>20km}/dt~=~1.263~\times~10^{-8}$ per year. \\
%=============================================

\subsection{Estimated crater densities and cratering chronology}
\textit{Third}, given the fitting ranges, we estimated the maximum crater densities for the earliest time possible. E.g., for Enceladus in the Saturnian system, we fitted for the collision after 100 Myr, then we could calculate the crater densities of the surface that is 4400 Myrs (4500 Myrs - 100 Myrs). \\

To perform the estimation, we need to combined three elements:
the fitting parameters from the deacy profile ($\tau$ and $\beta$), 
the normalized cumulative impact rate from the simulation ($dF(t=4500)/dt$), and
the actual impact rate onto the Enceladus ($dN_{D>20~km}/dt$). \\

We need to scale the decay profile's rate which is $dF(t=4500)/dt$ to match $dN_{D>20~km}/dt$, and create a ratio : 
\begin{eqnarray*}
\frac{dN}{dF} & = & \frac{dN_{D>20~km}}{dt}~\bigg/~\frac{dF(t=4500)}{dt}\\
& = & \frac{1.263 \times 10^{-8}~\rm per~year}{1.179 \times 10^{-14}~\rm per~year}\\
& = & 1.071 \times 10^{6}~\rm.
\end{eqnarray*}

The absolute cratering rate on Enceladus is :
\begin{eqnarray*}
\frac{dN_{D>20~\rm km}}{dt} &=& \frac{dN}{dF} \times \frac{dF_{4500}}{dt} \\ 
\frac{dN_{D>20~\rm km}}{dt} &=& \frac{dN}{dF} ~~ \beta~\tau^{-\beta}~t^{~\beta-1} \exp{\left[-\left(\frac{t}{\tau}\right)^\beta\right]}.\\
&&\\
\multicolumn{3}{l}{\rm Integrate both side by time,}\\
N_{D>20~\rm km} &=& \frac{dN}{dF}~\exp{\left[-\left(\frac{t}{\tau}\right)^\beta\right]}.
\end{eqnarray*}

We have the left-hand side as the estimated number of impacts ($N_{\rm D}$) on the whole Enceladus since ($4500-t$) million years old.
Our fitting for the decay profile of the Saturnian system is only valid up till 100 Myrs into the simulation, the earliest surface age we could infer is 4400 Mas for t=100 Myrs. From that, we calculated the estimated crater density ($n_{\rm D}$) of a 4400 Ma surface on Enceladus by further dividing the number of impact by the total surface area of Enceladus.

\begin{eqnarray*}
N_{D>20~\rm km} &=& \frac{dN}{dF}~\exp{\left[-\left(\frac{t}{\tau}\right)^\beta\right]}\\
&=&1.071 \times 10^{6}~\exp{\left[-\left(\frac{100}{0.602}\right)^{0.268}\right]}\\
&=& 20,912~\rm impacts.\\
\multicolumn{3}{l}{\rm Division over the spherical area of the satellites,}\\
n_{D>20\rm km} &=& N_{D>20~\rm km}~/~\rm Area \\
               &=& 20,912~/~798,648 ~\rm km^{2} \\
               &=& 0.0262~\rm impact~per~km^{2}.
\end{eqnarray*}

%======================================================
\subsection{The surface age}
\begin{figure*}[h!]
    \centering
    \resizebox{\hsize}{!}{\includegraphics{extra_fig/new_age.png}}
    \caption{}
    \label{fig:new_age}
\end{figure*}
\textit{Finally}, by scaling the decay profile of the collision on Saturn at t = 100 Myr (or 4400 Ma) with 0.0262, we construct the crater chronology of Enceladus since 4500 Ma. 
From the crater chronology, we derived the surface age by finding the time on the curves when the estimated crater density is same as the density we observed on Enceladus' terrain. In another word, we intercept the observed crater densities into the crater chronology to find the intercepting ages. \\

But, the crater chronology curves is not continuous, originally composed by several thousands or more collisions throughout 4500 Myrs. 
Instead of adopting a model (e.g., cumulative Weibull distribution) to draw a continuous curves and find the intercept, we simply search for the two closest data points that the observed crater density falls in, and use linear relationship between the two closet data points to derive the ages. (Please refer to figure~\ref{fig:new_age}). \\

This method could be more accurate in find the surface age. Because, firstly, often the model could not fit the entire decay profile very well, and the very few impacts in more recent time could not be traced decently by the model. This would problematic especially for young surface (e.g., less than 3 Ga). 
Secondary, the rapid decline in the curve at the beginning of the simulation (e.g., $<~$100 Myrs) would cause the model to sharply as age is push older (e.g., 4.4 Ga). Derived based on the model, the estimated crater densities for very old ages might be overestimated, leaving the surface age of ancient terrain underestimated. However, given the large change in crater densities relative to time at that ancient period, the resultant surface age would not different by much (also mentioned in \citet{Wong2020}). \\

The above steps was automatised using a code, we written in \textit{IDL} language. We demonstrated the manual calculation of surface age on a Enceladus' terrain as follows:\\

\textit{1.~} The estimated crater density for D$>20~$km at 100 Myr is 0.0262 per km$^{2}$. Express in the chronology plot (time v.s. $n_{\rm D}$), it is [100, 0.0262].
In the original normalized decay profile, it is [100, 0.0246] and the beginning of the curve is [0,1]. 
We scaled the decay profile at t = 100 Myr to match $n_{\rm D}$~=~0.025.
Shifting the entire profile up vertically, the beginning becomes [0.027, 1.063], and scaled profile, or now we could address as cratering chronology, corresponds to the expected crater densities on Enceladus for a surfaces that was form in different times.\\

\textit{2.~} The observed crater density for D$>20~$km is $8.50~\times~10^{-5}$ per km$^{2}$ for a surface on Enceladus \citep{Kirchoff2009}. We used codes to find the two closest points where the observed crater density lies in between, which is [1118.86, 0.00011] and [1293.75, 1e-7] (unfortunately, it's the last two data points). \\

\textit{3.~} Applied linear interpolation of the above two data points, we have [1161.95, 8.5E-5]. In another word, when the observed $n_{D>20~km}~=~8.5~\times~10^{-5}$, $t~=~1162$, which is \textbf{$\sim$3338 million years old}. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Problem with the above method}
\begin{figure*}[h!]
    \centering
    \resizebox{\hsize}{!}{\includegraphics{extra_fig/old_age.png}}
    \caption{}
    \label{fig:old_age}
\end{figure*}
We found the estimated $n_{D>20~km}$ = 0.0262~km$^{-2}$ on a 4.4 Ga Enceladus surface, with the new way to determine the impact flux backward in time. Just to recap, we deduce the incoming flux ($F_{\rm EC}$) with the current number of scatter disk objects ($N_{\rm SD}$), then using our latest decay profile to go backward in time to calculate the rate of impact. \\

The 0.0262~km$^{-2}$ is very different from the estimated crater density that we calculated in \citet{Wong2020} with Monte Carlo simulation and analytical calculation: 0.0828~km$^{-2}$ also for the crater with final size of 20~km in diameter, but on the surface formed in 4.5 Ga. Using the decay profile of collision on Saturn (Fig.~\ref{fig:sat}, especially judging by the upper-right panel), the cumulative impacts at 4.4 Ga is around $10^(-1.6) \approx 0.02476$ of those at the beginning, 4.5 Ga. Translating the latest $n_{D>20~km}$ at 4.4 Ga to 4.5 Ga, we have 0.0262/0.0247 = 1.063~km$^{-2}$ on Enceladus. This value is over an order of magnitude higher than what we found in \citet{Wong2020} (0.0828~km$^{-2}$). \\

If we apply the previous $n_{D>20~km}$ = 0.0828~km$^{-2}$ to anchor the decay profile for constructing the crater chronology of Enceladus, i.e., we scale the decay profile with [0,0.0828]. We have [616.94, 0.0828], means the surface ages is $4500-616.94$ = 3883 million years old. (Please refer to figure~\ref{fig:old_age})\\

\subsection{Remarks}
The new approach attempt to determine the estimated $n_{D>20~km}$ backward in time. The previous approach in \citet{Wong2020} calculate the estimated $n_{D>20~km}$ forward in time: starting from 4.5 Ga and go as the same direction as the simulation. Also in the previous approach, we calculate total number of impact on Enceladus with the initial number of planetesimals, 2.235$~\times~10^{12}$, derived from Monte Carlo experiment. But in the new approach we start with the current number of objects instead. \\

As seen from the above the new method give us the estimated $n_{D>20~km}$ an order of magnitude higher, thus compare with the same observed crater densities ($8.5~\times~10^{-5}$), the surface age determined with are several hundred million years younger. Given using the same $\tau$, $\beta$ and impact probability of Enceladus to calculate the $n_{D>20~km}$, the order of magnitude difference could be contributed by the uncertainties in calculating the incoming flux of the ecliptic comet crossing the giant planets orbit. Still need more thinking to understand, and more impact result to generate a more accurate fitting and chronologies. For example, the $8.5~\times~10^{-5}$ observed crater density we took from \citet{Kirchoff2009} lies in between the last two data points in our crater chronology (see \ref{fig:new_age}). Since the surface age is determined by linear interpolation, an extra collision adding in between the last two data point could have dramatically change ages. \\

%%%%%%%%%%%%%%% ending for now %%%%%%%%%%%%%%%5

\iffalse
1)
beta = 0.268; tau = 0.602. 
dF/dt = 0.268 * 0.602^(-0.268) * 4500^(0.268-1) * e^(-(4500/0.602)^0.268) =  1.179e-14 /yr. 
=B96*C96^(-B96)*4500^(B96-1)*EXP(-((4500/C96)^B96))

2) 
[ On Enceladus: ]
D_f = 20 km -->  D_i = 0.88 km
[ With N ~ D^0.7 from Nesvorny 2019]
N_sd(D_i>0.88km) = 2e9 / (0.88^0.7) = 2.19E9 
F_EC = 2.191E9 * 0.133 /Gyr = 0.291 /year.
dN/dt = 0.291 * 4.34E-8 = 1.263E-8 /year on Enceladus. 

%%%%%%%%%%%%%%%
D_f = 10 km -->  D_i = 0.41 km
N_sd(D_i>0.41km) = 2e9 / (0.41^0.7) = 3.718E9 
F_EC = 2.191E9 * 0.133 /Gyr = 0.494 /year.
dN/dt = 0.494 * 4.34E-8 = 2.144E-08 /year on Enceladus. 
%%%%%%%%%%%%%%%

3. 
dN/dF = 1.071E6                     %%% dN/dF = 1.806e6. 
N_(>20km;t=100) = 20,912            %%% N_10 = 35266
n_20km = 0.0262 km^-2 @4.4Ga         %%% n_10 = 0.044
       = 0.0262 * (10^1.6)           %%%      = 1.7517 @4.5Ga
       = 1.043 @4.5Ga                   

4. Compare with MC:
n_20km = 0.0828 @4.5Ga
[ fx=10^0=1 @4.5Ga;  fx=10^(-1.6)=0.025 ]
convert to 0.0828*0.025 =  0.002 km^-2 @4.4Ga
The calculation from MC is an order magnitude lower than the latest n_20. 

%%%%%%%%%%%%%%%

%Then # craters = 35266 and N_10 = 0.044 km^{-2} @ 4.4 Ga.
%Then at 4.5 Ga the density N_10 should be 0.044*10^(1.6) ~ 0.348. 
%For reference, the N_20 @ 4.5 ~ 0.08 km^{-2} so the expected N_10 ~
%N_20 * 2^3 ~ 0.66 km^{-2}.
%%%%%%%%%%%%%%%%%



%beta = 0.268; tau = 0.602. 
%Then dF/dt = 1.179e-14 /yr. 
%Then dN/dF = 1.806e6. 

%Then # craters = 35266 and N_10 = 0.044 km^{-2} @ 4.4 Ga.

%Then at 4.5 Ga the density N_10 should be 0.044*10^1.8 ~ 0.348. 
%For reference, the N_20 @ 4.5 ~ 0.08 km^{-2} so the expected N_10 ~
%N_20 * 2^3 ~ 0.66 km^{-2}.

\fi
